A Hybrid Data Cleaning Framework using Markov Logic Networks

With the increase of dirty data, data cleaning turns into a crux of data analysis. Most of the existing algorithms rely on either qualitative techniques (e.g., data rules) or quantitative ones (e.g., statistical methods). In this paper, we present a novel hybrid data cleaning framework on top of Markov logic networks (MLNs), termed as MLNClean, which is capable of cleaning both schema-level and instance-level errors. MLNClean mainly consists of two cleaning stages, namely, first cleaning multiple data versions separately (each of which corresponds to one data rule), and then deriving the final clean data based on multiple data versions. Moreover, we propose a series of techniques/concepts, e.g., the MLN index, the concepts of reliability score and fusion score, to facilitate the cleaning process. Extensive experimental results on both real and synthetic datasets demonstrate the superiority of MLNClean to the state-of-the-art approach in terms of both accuracy and efficiency.

==> MLN_Index_constrution.tex <==
%\section{Pre-processing}
%
%\begin{table}[t]
%\centering
%\caption{Example of grounding MLN rules using constants of $t_1$ in Table \ref{table:intro_sample}}
%\begin{tabular}{|c|l|l|} \hline
%\textbf{MLN rule}&\textbf{Grounding rule}&\textbf{Weight}\\      \hline
%\multirow{5}*{$\lnot$CT($v$) $\vee$ ST($v$)}&$\lnot$CT(DOTHAN) $\vee$ ST(AL)&$1/3$\\
%~&$\lnot$CT(DOTH) $\vee$ ST(AL)&$1/6$\\
%~&$\lnot$CT(BOAZ) $\vee$ ST(AL)&$1/3$\\
%~&$\lnot$CT(BOAZ) $\vee$ ST(AK)&$1/6$\\ \hline
%\end{tabular}
%\label{table:ground_rules}
%\end{table}
%
%The purpose of pre-processing is to transform different types of ICs into MLN rules for a unified expression, and ground these unified rules using constants in the input dataset. The term ground refers to a process that replace values with their corresponding constants in dataset. For instance, rule $r_1$ can be grounded using constants of $t_1$ in Table \ref{table:intro_sample}, the grounding results as show in table \ref{table:ground_rules}. After grounding process, we get a series of ground rules.

\section{MLN Index Construction}
\label{sec:construction}

\begin{figure*}
\centering
\includegraphics[width=7.2in]{fig/group}
\vspace*{-2mm}
\caption{Illustration of an MLN index over sample dataset.}
\label{fig:group}
%\vspace*{-10mm}
\end{figure*}

In this section, we describe an MLN index, a vital structure for the cleaning of MLNClean, which narrows errors search space by constructing a two-layer hash table.

%to (i) reduce error search range which contains two main operations, \emph{block} and \emph{group}, and (ii) calculate \emph{replacement score} for each ground rule as the basis for the subsequent data cleaning phase, denoted as the form of the index structure $\langle key, value\rangle$ where key represents a ground rule, value is the corresponding replacement score.


An MLN index is a two-layer hash table, with a set of \emph{blocks} in the first layer and a set of \emph{groups} in the second layer.
{\color{red}
All co-occurring data attribute values that ground MLN rules contain are finally divided into groups, we denote these data attribute values of each ground MLN rule as symbol $\gamma$, which is the smallest data unit supporting cleaning of multiple errors at once. Take the sample dataset in Table \ref{table:intro_sample} as an example, we depict the MLN index structure in Figure \ref{fig:group}.}

In the first layer, {\color{red}a set of $\gamma$ deriving from the same MLN rule are gathered in one \emph{block}}, that means, one block corresponds to one MLN rule.
Hence, the number of blocks is equivalent to the number of MLN rules.
%consists of two main operations: \emph{block} and \emph{group}. We introduce \emph{block} to divide the whole dataset into parts according to rules, each block contains a series of ground rules.
As shown in Figure \ref{fig:group}, there are three blocks $B_1, B_2$, and $B_3$ corresponding three rules $r_1, r_2$, and $r_3$ shown in Example~\ref{example:hai}, respectively.
%We select the attribute names related to the given rules, they are HN, CT, ST and PN. Thus, the dataset can be vertically divided into three blocks: $B_1$=\{CT, ST\}, $B_2$=\{HN, CT, ST, PN\}, $B_3$=\{CT, PN\}.



As known, each IC is composed of two parts, i.e., \emph{reason} part and \emph{result} part, and the \emph{reason} part determines the \emph{result} part.
In other words, there is no same reason to determine multiple different results.
Accordingly, within each block, we get {\color{red}$\gamma$s} with same reason part in one \emph{group}.
As a result, in the second layer, each block is divided into several groups, and {\color{red}$\gamma$s} within each group share one same reason part. In particular, for different types of rules, we decide the reason and result parts as follows.
First, for implication formulas (i.e., FDs and CFDs), they are in the form: $p_1$, $p_2$, $\dots$, $p_m$ $\Rightarrow$ $q_1$ $\vee$ $q_2$ $\vee\cdots\vee$ $q_n$.
The antecedent belongs to reason part, while the consequent pertains to result part.
In contrast, DC formulas have the following form: $\forall~t_1, \cdots, t_k ~\left( p_1 \wedge p_2 \wedge\cdots\wedge p_n \right)$.
{\color{blue} We simply treat the last predicate as result part, and the other predicates as reason part.}



%\emph{Block} operation divides the whole input dataset into several parts, the number of parts is determined by the number of rules.
%At first, we pick predicates of each rule which correspond to the attribute names of the input dataset, then we divide the whole dataset into parts according to the rules, each rule dominates a specific block. Each block contains a set of ground rules, and the content of each ground rule belongs to a specific tuple.



%Then we use the reason item as key to group GCs with the same reason value. It is easy to know that all GCs in the same group should have identical values but appears differently attributed to the existence of dirty data, i.e., the reason items have the same value while the result items have different values. Table \ref{table:4} show the group results based on the previous domain partition data in Table \ref{table:3}. For instance, considering Domain~2, there is a \emph{Group G=}\{$t_3$, $t_6$\} where GC of $t_3=$\{ELIZA, BOAZ, AL, 2565938310\}, GC of $t_6=$\{ELIZA, BOAZ, AL, 2567688400\} in this group, obviously there is a conflict at the value of attribute `PhoneNumber'.

%The overall algorithm is shown in Algorithm \ref{algorithm:domain}.

%\input{algorithm1}

%\begin{example}
%\label{example:block}
%Take the sample dataset in Table \ref{table:intro_sample} as an example. We select the attribute names related to the given rules, they are HN, CT, ST and PN. Thus, the dataset can be vertically divided into three blocks: $B_1$=\{CT, ST\}, $B_2$=\{HN, CT, ST, PN\}, $B_3$=\{CT, PN\}.
%%The partition result of blocks as shown in figure \ref{fig:block}.
%\end{example}

%\begin{figure}[t]
%\centering
%\includegraphics[width=3.3in]{fig/block}
%\caption{The block content of the sample dataset in Table \ref{table:intro_sample}}
%\label{fig:block}
%\end{figure}


%And each group can be treated as a candidate set where one of the ground rules is clean while the others with different values contain errors.



%\begin{example}
%We review the block results of Example \ref{example:block}, and execute \emph{Group} operation of each block. The block and group results as shown in Figure \ref{fig:group}. For instance, the block $B_1$ is divided into three groups $G_{11}$, $G_{12}$ and $G_{13}$, there is a group $G_{13}$ which contains three ground rules, $gr$=\{CT(BOAZ), ST(AK)\}, $gr$=\{CT(BOAZ), ST(AL)\} and $gr$=\{CT(BOAZ), ST(AL)\}. Obviously, there is a conflict at the value of attribute `ST'.
%\end{example}


%\begin{figure}[t]
%\centering
%\includegraphics[width=3.3in]{fig/domain_partition}
%\caption{Domain Partition}
%\label{fig:domain}
%end{figure}



%for the ground MLN rules with error(s) in reason part, they cannot be correctly classified to the corresponding groups, and thus becoming group outliers.
%Regarding this, \textsf{MLNClean} provides an outlier merging algorithm which attempts to push those outliers to the corresponding correct groups.

%It is worthwhile to mention that, for the ground MLN rules with error(s) in reason part, they cannot be correctly classified to the corresponding groups, and thus becoming group outliers.
%Regarding this, \textsf{MLNClean} provides an outlier merging algorithm which attempts to push those outliers to the corresponding correct groups.

%Group operation aggregates ground rules with the same reason. Nevertheless, considering such a ground rule $gr$, if dirty data appears on its reason part, it will not be properly classified.



%Thus, the purpose of outlier merging algorithm is to figure out outliers and put them into correct groups.

%\input{algorithm2}

%The pseudo code  of OM is shown in Algorithm \ref{algorithm:outlierMerging}.

%After figure out outlier group, we need to put them into correct groups. In MLNClean, we compare each outlier group $OG$ with other regular groups in $\mathbb{G}_i - OG$, and put all outliers within the same outlier group into a regular group which is most similar to this outlier group (Line 7-8). Since it is hard to compute the similarity of two groups, we use a $gr$ with the largest number in the group to represent this whole group, thus the similarity between two groups is transformed to the similarity between two $gr$s. We use the distance metrics that introduced before (see Definition \ref{equation:replace_score}) to represent the similarity.


{\color{red}We analyse the time complexity of MLN index structure in each step. In order to divide the whole dataset into blocks according to the input ICs, we need to iterate through each tuple in the dataset to find those attributes of tuple that match predicates of rules. The time complexity of this step is $O(|B| \times |T|)$, where $|B|$ is the number of blocks, which is equal to the number of rules, $|T|$ is the number of tuples. Then, we traverse each block once to put $\gamma$s with the same reason part into a group, the time complexity of this step is $O(|B| \times |T|)$ as well. Thus, the total time complexity of MLN index structure is $O(|B| \times |T|)$.
}

%In order to find each $G_{min}$ in its corresponding block, we need to spend $|\mathbb{G}_i|$ times, thus in the worst case, the time complexity of our proposed outlier merging algorithm is $O(|B||\mathbb{G}_i|^2)$, and in the best case, the time complexity is $O(|B||\mathbb{G}_i|)$.






%In general, we can use Markov inference to compute the most probable probability of each value. However, our purpose is to compute the joint distribution of ground rules while Markov inference can only reason probabilistically about a single attribute value itself, thus it is hard to use native Markov inference to find the most probable joint distribution of ground rules.
%In view of the above-mentioned fact, we use MLN weight learning instead. And we explain how to convert Markov inference equation to weight learning equation as follows:
%In \textsf{MLNClean}, we change MLN rules to ground  MLN rules as the target that weight learning needs to train.
%Thus, from Equation \ref{equation:markov_prob},
%\begin{equation}
%\begin{aligned}
%\Pr(\gamma)& = \frac{1}{Z} e^{\sum_{i=1}^{N} w_i n_i(\gamma)}   \\
%%   &=\frac{1}{Z} {\rm exp} \left(\sum_{i=1}^{n} w_i f_i(x) \right)   \\
%%   &=\frac{1}{Z} {\rm exp} \left(\sum_{i=1}^{n} w_i \right)~~~~\because f_i(x)=1  \\
%\ln \Pr(\gamma)& = \ln(\frac{1}{Z} \cdot e^{w_i}) = w_i - \ln Z \\
%\end{aligned}
%\end{equation}
%where $\ln Z$ is a constant, and $\ln\Pr(\gamma)$ is a monotonically increasing function which means the greater weight, the higher probability. Therefore, the inference process can be replaced by MLN weight learning process in \textsf{MLNClean}, and we use weight learning process to find the most probable probability of each ground rule.


%In order to figure out which ground MLN rule is clean in each group, and try to preserve as many ground rules as possible so as to have a minimal impact on the dataset.
%\textsf{MLNClean} treats all ground rules within a group as a candidate set of clean data, and then uses \emph{replacement score} to represent the clean possibility of each ground rule in a group.
%Ultimately, \textsf{MLNClean} picks the one which has the maximal replacement score as the clean ground rule while the others are dirty.


%In each group, at first MLNClean regard the first GC as dirty clause and treat the other GCs differ from the first one in value as its candidates, hereafter calculate the similarity between dirty clause and each of its candidate, and use MLN weight learning method to compute their joint distribution probability. Ultimately, MLNClean record the maximal replacement score candidate as a replacement of this dirty clause, then MLNClean move to the next GC and repeat the above operations until all GCs being traversed. Thus, MLN index construction is finished, and output all GCs with their most probable replacement for the preparation of the following cleaning process.



%After all GCs get their most probable replacement, MLNClean sort these replacements according to how many times they appear, and choose the one with the most frequent occurrences as the replacement of the whole group.




==> algorithm-crowdsourcing.tex <==
\begin{algorithm}[t]
\label{algorithm:crowsourcing}
%    \SetAlgoNoLine  %去掉之前的竖线
\caption{A Crowdsourcing based Abnormal Group Process}
    \KwIn{$\rm Dataset\;\emph S$, $\rm Set\;of\;Rules\;\emph{R}$}
    \KwOut{a set of blocks $B$}
        %List $B$ = new List(\emph{R}.size)\;
        \For{$each\;r_i\in R$}
        {
            
            
        }
        return $B$\;
\end{algorithm}


==> algorithm1.tex <==
%\begin{algorithm}[t]
%\label{algorithm:domain}
%%    \SetAlgoNoLine  %去掉之前的竖线
%\caption{Partition dataset into blocks}
%    \KwIn{$\rm Dataset\;\emph S$, $\rm Set\;of\;Rules\;\emph{R}$}
%    \KwOut{a set of blocks $B$}
%        %List $B$ = new List(\emph{R}.size)\;
%        \For{$each\;r_i\in R$}
%        {
%            Distinguish \emph{reason} and \emph{result} parts in each $r_i$\;
%            %Split \emph{values} in \emph{Tuple} by attributes;\\
%            \For{$each\;Tuple\;in\;S$}
%            {
%                gr = new GR(); //Init an empty ground rules\\
%                $v_l\leftarrow$ select \emph{values} belong to \emph{reason} part of $r_i$\;
%                $v_r\leftarrow$ select \emph{values} belong to \emph{result} part of $r_i$\;
%                %$Tr_i\leftarrow$ select \emph{values} belong to $r_i$\;
%                gr.putValue($v_l$, $v_r$)\;
%                $B_i$.add(gr)\;
%            }
%            $B$.add($B_i$)\;
%
%        }
%        return $B$\;
%\end{algorithm}


==> algorithm2.tex <==
\begin{algorithm}[t]\small
\label{algorithm:outlierMerging}
\SetNlSty{small}{}{:}
%\SetNlSkip{4mm}
\LinesNumbered
\DontPrintSemicolon
\caption{Outlier Merging Algorithm}
    \KwIn{Set of blocks $B$, set of groups $\mathbb{G}$}
    \KwOut{Set of groups $\mathbb{G}$}
        \For{$each\;B_i\in B$}
        {
            $\mathbb{G}_i \leftarrow$ get a set of groups belong to $B_i$\;
            \For{$each\;G_{ij}\in \mathbb{G}_i$}
            {
                $OG=\varnothing$ // Initial outlier group $OG$\;
                \If{$N(G_{ij})$ $< \tau$}{
                    $OG = G_{ij}$\;
                    %$G_{min}\leftarrow$ find $d_{min}$ between $OG$ and other groups in $\mathbb{G}_i - OG$\;
                    $G_{min}\leftarrow$ find the group most similar to $OG$\;
                    $G_{min}$.addAll($OG$)\;
                    $\mathbb{G}_i$.update($G_{min}$)\;
                }
            }
        }
        return $\mathbb{G}$\;
\end{algorithm}

